Adaptive Target Tracking Using Retrospective Cost Input Estimation

Target tracking of surrounding vehicles is essential for collision avoidance in autonomous vehicles. Our approach to target tracking is based on causal numerical differentiation on relative position data to estimate relative velocity and acceleration. Causal numerical differentiation is useful for a wide range of estimation and control problems with application to robotics and autonomous systems. The present paper extends prior work on causal numerical differentiation based on retrospective cost input estimation (RCIE). Since the variance of the input-estimation error and its correlation with the state-estimation error (the sum of the variance and the correlation is denoted as $\widetilde{V}$) used in the Kalman filter update are unknown, the present paper considers an adaptive discrete-time Kalman filter, where $\widetilde{V}_k$ is updated at each time step $k$ to minimize the difference between the sample variance of the innovations and the variance of the innovations given by the Kalman filter. The performance of this approach is shown to reach the performance of numerical differentiation based on RCIE with the best possible fixed value of $\widetilde{V}_k$. The proposed method thus eliminates the need to determine the best possible fixed value for $\widetilde{V}_k$. Finally, RCIE with an adaptive Kalman filter is applied to target tracking of a vehicle using simulated data from CarSim.

==> old_files/zDiscussions.tex <==




Hi Shashank,

Can you pls help me insert the references for the introduction?

Thanks


 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Is there only 1 paper on HGO?
We only looked at one paper. 



Do we have other references on sliding mode?

Yes, I added the other one.
what about that huge report we found online?  can that one be cited?
it had numerical techniques I think
Are you taking about the one that Dogan suggested? 
no I dont think so, I think I found it not sure, let me look
148 pages I just sent it to you
Ok, we can add that. They talk about linear, sliding-mode based, adaptive, Kalman, and ALIEN differentiators. Need to read what "ALIEN" is? 

no idea





Do we have other reference on SG?
i will try to find more and add it








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Do you have references on adaptive KF?

There was one. [13] one. I. Yaesh and U. Shaked, “Simplified adaptive estimation,” Syst. Con-
trol. Lett., vol. 57, pp. 49–55, 2008.
we added this and other paeprs too


do you have a few more on adative KF?

are those cited in the introduction now?  follow me please

what about the Junkins paper and other papers we found?

junkins is not a Kalman one. They are doing optimization



Please add any references that you feel are relevant

Do you have more adaptive KF references?


here


I think the intro is in pretty good shape.  I will refine it later.

what are you working on now in the paper?

plase write the contents paragraph

?? oh ok. 
look at the end of the introduction


you can add any other references you find but we probably have enough.

As you can see we missed that IJC special issue although we did have ONE of those references

Yes. Yes wee saw with acc paper.

we should not miss references------reviewers get upset right?

you should keep doing searches just to be sure

ok, I will check back later tonite

You can work on this tomorrow, right? 

yes, I can. I will try to finish it by monday evening or afti. Ok. Can you remove the extra content from introduction? or Should I? Oh you did. I just recompile. 

ok, ttyl thanks
Thanks

let me check it I thought I already did that rec oinpiuline


myabe you can submit it monday nite, ok?

ok, good.  I will write the conclusions now and check back later thanks






Section 5 and 6




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Summary from meeting 8/18/22




We should construct the closed loop system and look at the bode plots.  If y is a sinusoid or sum of sinusoids, we should see if we get approximately 90 deg of phase lead and the correct gain at each sinusoidal frequency.


We should do this over a range of values of nc.  If nc is larger than needed, the hope is that RCIE will still arrive at the correct gain and phase.

This can be messed up by V1 and V2.  We can use the true V2, but there is no true V1.

RLS is never perfectly accurate due to the regularization (Brian had a paper on this).

Everything I have said so far is withOUT forgetting.  We may bring in forgetting later and it is mainly needed when there is an abrupt change although it might have benefits even without abrupt changes.  But it also causes other problems.  I am thinking of adaptive forgetting.


Sneha can do all of these things for integration.

After these things are tested, we can replace KF with RCSE.  The advantage is that we dont need to specify V1 and V2.

If that looks promising we can consider a combined RCIE/RCSE------perhaps one RLS or perhaps more closely merged.  Maybe that will be easy, I have no idea.

Please add any ideas here.  Thanks














